Provably Efficient $Q$-learning with Function Approximation via Distribution Shift Error Checking Oracle

$Q$-learning with function approximation is one of the most popular methods in reinforcement learning. Though the idea of using function approximation was proposed at least 60 years ago, even in the simplest setup, i.e, approximating $Q$-functions with linear functions, it is still an open problem on how to design a provably efficient algorithm that learns a near-optimal policy. The key challenges are how to efficiently explore the state space and how to decide when to stop exploring in conjunction with the function approximation scheme. The current paper presents a provably efficient algorithm for $Q$-learning with linear function approximation. Under certain regularity assumptions, our algorithm, Difference Maximization $Q$-learning (DMQ), combined with linear function approximation, returns a near-optimal policy using a polynomial number of trajectories. Our algorithm introduces a new notion, the Distribution Shift Error Checking (DSEC) oracle. This oracle tests whether there exists a function in the function class that predicts well on a distribution $\mathcal{D}_1$, but predicts poorly on another distribution $\mathcal{D}_2$, where $\mathcal{D}_1$ and $\mathcal{D}_2$ are distributions over states induced by two different exploration policies. For the linear function class, this oracle is equivalent to solving a top eigenvalue problem. We believe our algorithmic insights, especially the DSEC oracle, are also useful in designing and analyzing reinforcement learning algorithms with general function approximation.

==> algo.tex <==
We first present the algorithm for MDP with sparse reward, i.e., $Q(x,a) \in \left\{0,1\right\}$ and unique.
This assumption implies the following proposition.
\begin{prop}
For every $h$, there exists a sequence of actions $a_1,\ldots,a_h$ such that $Q(x_h,a) = 1$ for some $a \in \actions$.
\end{prop}
Thus it is enough to main paths (sequence of actions).
Based on this observation, we can derive the following algorithm.

\begin{algorithm}[t]
	\floatname{algorithm}{Algorithm}
	\caption{Algorithm for $0,1$ Reward}
	\label{algo:stochastic}
	\begin{algorithmic}[1]
		\Statex \textbf{Output}: $V_H$
		\For{$h=1:H$}
		\State Initialize $V_h = \phi$.
		\State Initialize $S = \phi$.
		\For{$v_h \in V_{h-1}$}
			\For {$a \in \actions$}
				\State Execute $a \circ v_h$ and observe $x$.
				\State if $x$ is NOT in the linear span of $S$, add $x$ to $S$ and add $a \circ v_h$ to $V$.
			\EndFor
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}




%\begin{algorithm}[t]
%	\floatname{algorithm}{Algorithm}
%	\caption{Stochastic Contextual Decision Process using State-Action Pair Prediction}
%	\label{algo:stochastic}
%	\begin{algorithmic}[1]
%		\Statex \textbf{Input}: $N_{exp}$: number of data to learn $\hat{g}$, $N_{cluster}$: number of data to find a representation of each state through clustering, $N_{p}$: number of data  $\states_0 = \left\{s_{start}\right\}$,
%		$\tau$: thresholding parameter to do identity test.
%		$\tau_1$: thresholding parameter to determine whether a state is stored or ignored.
%		\Statex \textbf{Output}: $\widehat{\states}_1,\ldots,\widehat{\states}_H$ where element in $\widehat{\states}_h$ is the state represented by a $\abs{\widehat{\states}_{h-1}}K$ dimensional vector. $\widehat{P}_1,\ldots,\widehat{P}_H$: transition probability tensor $\widehat{P}(s'|s,a) \in \mathbb{R}$.
%
%		\For{$h=1:H$}
%		\State \simon{Learn the prediction function.}
%		\State Denote $\Pi_{h-1} = \left\{\hat{\pi}_{\hat{s}}\right\}_{\hat{s} \in \widehat{\states}_{h-1}}$ (	For $h=1$, $\hat{\pi}_{\hat{s}_{start}}$ represents the known starting state).
%		\State Use $\widehat{P}$ to estimate the probability of reaching each state $\left\{\hat{P}^{\Pi_{h-1}}(\hat{s})\right\}_{\hat{s} \in \widehat{\states}_{h-1}}$ if we use policy $\unif[\Pi_h]$.
%		\State Define policy $\pi_h \triangleq \unif[\mathcal{A}] \circ \unif [\Pi_h]$ and $\vect{p}_h = \left(\hat{P}^{\Pi_{h-1}}(\hat{s},a)\right)_{\hat{s} \in \widehat{\states}_{h-1}, a\in \actions}$ with $\hat{P}^{\pi_h}(\hat{s},a) = \frac{\hat{P}(\hat{s})}{K}$.
%		\State Execute policy $\pi_h$ to get $N_{exp}$ samples and stored in a data set $D_h$. Each sample is a tuple $\left(\hat{s},a,x'\right)_{\hat{s} \in \widehat{\states}_{h-1}, a \in \mathcal{A}, x' \in \contexts_{h}}$.
%		\State Use Oracle~\ref{defn:weighted_erm} with input $D_h$ and $\vect{p}_h$ to learn $\hat{g}_h$.
%		\State \simon{Learn the representation}
%		\State Execute $\pi_h$ for $N_{cluster}$ times and collect data $D_h^{cluster} = \left\{\hat{g}_h(x_i')\right\}_{i=1}^{N_{cluster}}$ where $x_i'$s are contexts at level $h$.
%		\State Use Algorithm~\ref{algo:find_representation} with input $D_h^{cluster}$ and $\tau$ to learn $\widehat{\states}_h$.
%		\State Define the decoding function $\hat{f}_h$ according to Equation~\eqref{eqn:decoding_function}.
%		\State \simon{Learn the transition probability}
%		\State Execute the policy $\pi_h$ for $N_p$ times and put every tuple $\left(s,a,\hat{f}_h(x')\right)_{s \in \widehat{\states}_{h-1}, a \in \actions, x' \in \widehat{\states}_{h}}$ in $D_p$.
%		\State Use $D_p$ to compute $\widehat{P}_h\left(\widehat{\states}_{h}|\widehat{\states}_{h-1},\actions\right)$.
%		%		\State \simon{Ignore states with low maximum reaching probability}
%		%		\For{$s \in \widehat{\states}_{h}$}
%		%			\State Use dynamic programming to compute $\hat{\pi}_{\hat{s}} = \argmax_{\pi} \widehat{P}^{\pi}(\hat{s})$
%		%			\If{$\hat{P}^{\hat{\pi}_{\hat{s}}}(\hat{s}) \le \tau_1$}
%		%				\State $\widehat{S}_h = \widehat{S}_h \setminus \{\hat{s}\}$.
%		%			\EndIf
%		%		\EndFor
%		%		\State Update the decoding function $\hat{f}_h$ according to Equation~\eqref{eqn:decoding_function}.
%		\EndFor
%	\end{algorithmic}
%\end{algorithm}


